VaultDB: A Real-World Pilot of Secure Multi-Party Computation within a Clinical Research Network

Electronic health records represent a rich and growing source of clinical data for research. Privacy, regulatory, and institutional concerns limit the speed and ease of sharing this data. VaultDB is a framework for securely computing SQL queries over private data from two or more sources. It evaluates queries using secure multiparty computation: cryptographic protocols that evaluate a function such that the only information revealed from running it is the query answer. We describe the development of a HIPAA-compliant version of VaultDB on the Chicago Area Patient Centered Outcomes Research Network (CAPriCORN). This multi-institutional clinical research network spans the electronic health records of nearly 13M patients over hundreds of clinics and hospitals in the Chicago metropolitan area. Our results from deploying at three health systems within this network show its efficiency and scalability for distributed clinical research analyses without moving patient records from their site of origin.

==> background.tex <==

\section{Background}

We will now review the landscape in which we conducted this work and highlight key challenges in this space.

\subsection{Regulatory Landscape} 
\label{sec:regs}
The goal of this research is to facilitate clinical research over diverse patient populations to enable new precision medicine for individuals and faster, more accurate public health surveillance.  We aim to do this in settings where conventional data sharing agreements are either not possible or too onerous to be actionable.  Secure querying of EHRs will enable researchers and clinicians to quickly identify healthcare interventions and evaluate their potential efficacy for precision medicine even if the relevant patient records are fractured over two or more sites.  Supporting fractured care is especially important for more vulnerable community members such as individuals experiencing homelessness.  

At the time of this writing, conducting research of this kind is quite challenging.  The federal regulations and guidance for data access in clinical research were created before the big data era. In the US, they largely come in two forms. First, the Health Insurance Portability and Accountability Act (HIPAA) of 1996 is the main legislative driver of patient privacy. It informs how healthcare teams for a patient share data amongst themselves. Second, investigators perform research under the “Common Rule”, an ethical standard that defines how they protect participants in a research study. It requires that studies implement informed consent for all participants and the oversight of the Institutional Review Board (IRB) at the investigator’s home institution for all federally-funded research.  A CRN usually stands up shared IRB infrastructure so the data partners may delegate to it for authorizing individual studies.

When investigators wish to conduct research over electronic health records from multiple health- care institutions, they start by establishing data use agreements~\cite{malin2010technical}. Here, each institution, or data partner, remains responsible maintaining compliance with all applicable laws and regulations for their data. These agreements protect patient confidentiality. They also specify the mechanisms for data sharing, the roles and responsibilities of all participants, and acceptable use of shared data. Moreover, investigators conducting studies on this data agree to not attempt to re-identify study participants.  When a healthcare organization negotiates a data use agreement with these networks, it often takes months or more of committee and legal work. Hence, it can take many years for a network to build up a diverse cohort of patients for precision medicine research.   Further complicating this endeavor, this research is subject to a witch’s brew of complex, partially overlapping regulations that vary by jurisdiction, divergent interpretations by stakeholders, and by the contents of the data itself. There are many valid concerns about patient privacy in this research, and we, with numerous others, are working on a principled approach to addressing them. A second, related concern is building an ecosystem of support to encourage individuals and healthcare institutions to share their data for research. 


In this pilot, we work within the Chicago Area Patient-Centered Outcomes Research Network or CAPriCoRN.  This CRN spans 10 major healthcare institutions.  In our study, we deployed VaultDB at two academic medical centers: Rush University and Northwestern Medicine and one network of community health centers, Alliance of Chicago.  


\subsection{Secure Multiparty Computation}
VaultDB uses secure multiparty computation to evaluate its queries securely by passing encrypted messages among the data partners.   Its cryptographic backend is powered by EMP Toolkit~\cite{emp-toolkit}.  \emp~\cite{emp-toolkit} stands for Efficient Multi-Party computation toolkit.  This open-source project was started in 2016 by Xiao Wang and Jon Katz and it is actively maintained by them. The toolkit is developed to address two goals: 
1) provide an easy way for researchers to build efficient cryptographic
prototypes; 2) provide a user-friendly interface for non-cryptographic developers
to write privacy-preserving applications.
It consist of multiple libraries organized in three layers:
\begin{enumerate}
\item {\it Basic non-interactive primitives.} \emp provides interfaces and efficient 
hardware-accelerated implementation of commonly used cryptographic primitives,
including encryption, public-key cryptography, hashing, garbling, as well as an
on-the-fly circuit compiler.
\item {\it Basic interactive primitives.} \emp also provides a rich set of basic
interactive primitives that are useful for constructing secure multi-party computation
protocols, e.g., oblivious transfer protocols.
\item {\it Secure multi-party computation protocols.} Currently, \emp supports
a rich set of protocols for secure multi-party computation, including implementations for different 
numbers of participants and security models. In particular, it offers semi-honest
two-party computation, malicious two-party computation protocol,
as well as malicious multi-party computation protocol.  We deploy the semi-honest protocols in this study.
\end{enumerate}
    

==> bibitems.tex <==
% bbl / $ biblatex auxiliary file $
% $ biblatex bbl format version 3.1 $
% Do not modify the above lines!
%
% This is an auxiliary file used by the 'biblatex' package.
% This file may safely be deleted. It will be recreated by
% biber as required.
% 
\begingroup
\makeatletter
\@ifundefined{ver@biblatex.sty}
  {\@latex@error
     {Missing 'biblatex' package}
     {The bibliography requires the 'biblatex' package.}
      \aftergroup\endinput}
  {}
\endgroup


\refsection{0}
  \datalist[entry]{none/global//global/global}
    \entry{hipaa}{misc}{}
      \name{author}{1}{}{%
        {{hash=b5b66ca68cc9f1797b1d5996fa186ecd}{%
           family={{Centers for Medicare \& Medicaid Services}},
           familyi={C\bibinitperiod}}}%
      }
      \strng{namehash}{b5b66ca68cc9f1797b1d5996fa186ecd}
      \strng{fullhash}{b5b66ca68cc9f1797b1d5996fa186ecd}
      \strng{bibnamehash}{b5b66ca68cc9f1797b1d5996fa186ecd}
      \strng{authorbibnamehash}{b5b66ca68cc9f1797b1d5996fa186ecd}
      \strng{authornamehash}{b5b66ca68cc9f1797b1d5996fa186ecd}
      \strng{authorfullhash}{b5b66ca68cc9f1797b1d5996fa186ecd}
      \field{sortinit}{1}
      \field{sortinithash}{4f6aaa89bab872aa0999fec09ff8e98a}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{title}{{The Health Insurance Portability and Accountability Act of 1996 (HIPAA)}}
      \field{year}{1996}
    \endentry
    \entry{hitech}{article}{}
      \name{author}{1}{}{%
        {{hash=a55dfabd37fbff7cad6cef5d92c4f386}{%
           family={Blumenthal},
           familyi={B\bibinitperiod},
           given={David},
           giveni={D\bibinitperiod}}}%
      }
      \strng{namehash}{a55dfabd37fbff7cad6cef5d92c4f386}
      \strng{fullhash}{a55dfabd37fbff7cad6cef5d92c4f386}
      \strng{bibnamehash}{a55dfabd37fbff7cad6cef5d92c4f386}
      \strng{authorbibnamehash}{a55dfabd37fbff7cad6cef5d92c4f386}
      \strng{authornamehash}{a55dfabd37fbff7cad6cef5d92c4f386}
      \strng{authorfullhash}{a55dfabd37fbff7cad6cef5d92c4f386}
      \field{sortinit}{2}
      \field{sortinithash}{8b555b3791beccb63322c22f3320aa9a}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{journaltitle}{New England Journal of Medicine}
      \field{number}{5}
      \field{title}{Launching {HITECH}}
      \field{volume}{362}
      \field{year}{2010}
      \field{pages}{382\bibrangedash 385}
      \range{pages}{4}
    \endentry
    \entry{kho2014capricorn}{article}{}
      \true{moreauthor}
      \true{morelabelname}
      \name{author}{10}{}{%
        {{hash=20a18291bfb11419b26ee7fa7e757f66}{%
           family={Kho},
           familyi={K\bibinitperiod},
           given={Abel\bibnamedelima N},
           giveni={A\bibinitperiod\bibinitdelim N\bibinitperiod}}}%
        {{hash=8c8a54e945df44935c23f00dda2cafbf}{%
           family={Hynes},
           familyi={H\bibinitperiod},
           given={Denise\bibnamedelima M},
           giveni={D\bibinitperiod\bibinitdelim M\bibinitperiod}}}%
        {{hash=b94ece5719ca6bb41b96b5b30667bcdc}{%
           family={Goel},
           familyi={G\bibinitperiod},
           given={Satyender},
           giveni={S\bibinitperiod}}}%
        {{hash=06ed39f4441faa7777730908e1b36bed}{%
           family={Solomonides},
           familyi={S\bibinitperiod},
           given={Anthony\bibnamedelima E},
           giveni={A\bibinitperiod\bibinitdelim E\bibinitperiod}}}%
        {{hash=03009df21866ed0f77d1a48f332e4b75}{%
           family={Price},
           familyi={P\bibinitperiod},
           given={Ron},
           giveni={R\bibinitperiod}}}%
        {{hash=f7c0e60f1d6c58ff6c55aa75880e3ac4}{%
           family={Hota},
           familyi={H\bibinitperiod},
           given={Bala},
           giveni={B\bibinitperiod}}}%
        {{hash=ee11b811b03092bde56ac14bde84ca85}{%
           family={Sims},
           familyi={S\bibinitperiod},
           given={Shannon\bibnamedelima A},
           giveni={S\bibinitperiod\bibinitdelim A\bibinitperiod}}}%
        {{hash=5d19806df471e5ee94c2033036971e18}{%
           family={Bahroos},
           familyi={B\bibinitperiod},
           given={Neil},
           giveni={N\bibinitperiod}}}%
        {{hash=d8cdf6b9237ab298ee6cced64296528f}{%
           family={Angulo},
           familyi={A\bibinitperiod},
           given={Francisco},
           giveni={F\bibinitperiod}}}%
        {{hash=9533a43ff9aef61211dfcb9eae374860}{%
           family={Trick},
           familyi={T\bibinitperiod},
           given={William\bibnamedelima E},
           giveni={W\bibinitperiod\bibinitdelim E\bibinitperiod}}}%
      }
      \list{publisher}{1}{%
        {BMJ Publishing Group}%
      }
      \strng{namehash}{5bb064c342c4832e8537c7e9f794cdce}
      \strng{fullhash}{1d5904dec9b8590c4ef3838943bfbe45}
      \strng{bibnamehash}{5bb064c342c4832e8537c7e9f794cdce}
      \strng{authorbibnamehash}{5bb064c342c4832e8537c7e9f794cdce}
      \strng{authornamehash}{5bb064c342c4832e8537c7e9f794cdce}
      \strng{authorfullhash}{1d5904dec9b8590c4ef3838943bfbe45}
      \field{extraname}{1}
      \field{sortinit}{3}
      \field{sortinithash}{ad6fe7482ffbd7b9f99c9e8b5dccd3d7}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{journaltitle}{Journal of the American Medical Informatics Association}
      \field{number}{4}
      \field{title}{CAPriCORN: Chicago area patient-centered outcomes research network}
      \field{volume}{21}
      \field{year}{2014}
      \field{pages}{607\bibrangedash 611}
      \range{pages}{5}
    \endentry
    \entry{capricorn}{misc}{}
      \name{author}{1}{}{%
        {{hash=bee7ccdd4f05dbdfa8e35fbd72dac849}{%
           family={{Chicago Area Patient-Centered Outcomes Research Network}},
           familyi={C\bibinitperiod}}}%
      }
      \strng{namehash}{bee7ccdd4f05dbdfa8e35fbd72dac849}
      \strng{fullhash}{bee7ccdd4f05dbdfa8e35fbd72dac849}
      \strng{bibnamehash}{bee7ccdd4f05dbdfa8e35fbd72dac849}
      \strng{authorbibnamehash}{bee7ccdd4f05dbdfa8e35fbd72dac849}
      \strng{authornamehash}{bee7ccdd4f05dbdfa8e35fbd72dac849}
      \strng{authorfullhash}{bee7ccdd4f05dbdfa8e35fbd72dac849}
      \field{sortinit}{3}
      \field{sortinithash}{ad6fe7482ffbd7b9f99c9e8b5dccd3d7}
      \field{labelnamesource}{author}
      \field{howpublished}{\url{https://www.capricorncdrn.org/about/}}
      \field{note}{Accessed: 2022-02-25}
    \endentry
    \entry{kho2015design}{article}{}
      \true{moreauthor}
      \true{morelabelname}
      \name{author}{10}{}{%
        {{hash=20a18291bfb11419b26ee7fa7e757f66}{%
           family={Kho},
           familyi={K\bibinitperiod},
           given={Abel\bibnamedelima N},
           giveni={A\bibinitperiod\bibinitdelim N\bibinitperiod}}}%
        {{hash=d6a5478e8618474db2faf9db9b1828e8}{%
           family={Cashy},
           familyi={C\bibinitperiod},
           given={John\bibnamedelima P},
           giveni={J\bibinitperiod\bibinitdelim P\bibinitperiod}}}%
        {{hash=04040fd5e4bb8058acaeb3840a13db55}{%
           family={Jackson},
           familyi={J\bibinitperiod},
           given={Kathryn\bibnamedelima L},
           giveni={K\bibinitperiod\bibinitdelim L\bibinitperiod}}}%
        {{hash=cf1090414d9824d88edc18ab287e6a04}{%
           family={Pah},
           familyi={P\bibinitperiod},
           given={Adam\bibnamedelima R},
           giveni={A\bibinitperiod\bibinitdelim R\bibinitperiod}}}%
        {{hash=b94ece5719ca6bb41b96b5b30667bcdc}{%
           family={Goel},
           familyi={G\bibinitperiod},
           given={Satyender},
           giveni={S\bibinitperiod}}}%
        {{hash=556c150a99831e1091334bbd846a73c9}{%
           family={Boehnke},
           familyi={B\bibinitperiod},
           given={Jörn},
           giveni={J\bibinitperiod}}}%
        {{hash=c26c1f9ee1b3f07a1b236c09ce64fb60}{%
           family={Humphries},
           familyi={H\bibinitperiod},
           given={John\bibnamedelima Eric},
           giveni={J\bibinitperiod\bibinitdelim E\bibinitperiod}}}%
        {{hash=fdf5013c4b6adb570f774dc5710909a5}{%
           family={Kominers},
           familyi={K\bibinitperiod},
           given={Scott\bibnamedelima Duke},
           giveni={S\bibinitperiod\bibinitdelim D\bibinitperiod}}}%
        {{hash=3b20430f1c7de4a465a16ee6de83090e}{%
           family={Hota},
           familyi={H\bibinitperiod},
           given={Bala\bibnamedelima N},
           giveni={B\bibinitperiod\bibinitdelim N\bibinitperiod}}}%
        {{hash=ee11b811b03092bde56ac14bde84ca85}{%
           family={Sims},
           familyi={S\bibinitperiod},
           given={Shannon\bibnamedelima A},
           giveni={S\bibinitperiod\bibinitdelim A\bibinitperiod}}}%
      }
      \list{publisher}{1}{%
        {Oxford University Press}%
      }
      \strng{namehash}{5bb064c342c4832e8537c7e9f794cdce}
      \strng{fullhash}{4ac60e0454c255efc2b9324b2d81e900}
      \strng{bibnamehash}{5bb064c342c4832e8537c7e9f794cdce}
      \strng{authorbibnamehash}{5bb064c342c4832e8537c7e9f794cdce}
      \strng{authornamehash}{5bb064c342c4832e8537c7e9f794cdce}
      \strng{authorfullhash}{4ac60e0454c255efc2b9324b2d81e900}
      \field{extraname}{2}
      \field{sortinit}{4}
      \field{sortinithash}{9381316451d1b9788675a07e972a12a7}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{journaltitle}{Journal of the American Medical Informatics Association}
      \field{number}{5}
      \field{title}{Design and implementation of a privacy preserving electronic health record linkage tool in Chicago}
      \field{volume}{22}
      \field{year}{2015}
      \field{pages}{1072\bibrangedash 1080}
      \range{pages}{9}
    \endentry
    \entry{mays2016evaluation}{article}{}
      \name{author}{8}{}{%
        {{hash=c3050ecadec26e44a6a7746a39ddfe39}{%
           family={Mays},
           familyi={M\bibinitperiod},
           given={James\bibnamedelima A},
           giveni={J\bibinitperiod\bibinitdelim A\bibinitperiod}}}%
        {{hash=04040fd5e4bb8058acaeb3840a13db55}{%
           family={Jackson},
           familyi={J\bibinitperiod},
           given={Kathryn\bibnamedelima L},
           giveni={K\bibinitperiod\bibinitdelim L\bibinitperiod}}}%
        {{hash=ffa05d4a860761e79b6f1690580b05a5}{%
           family={Derby},
           familyi={D\bibinitperiod},
           given={Teresa\bibnamedelima A},
           giveni={T\bibinitperiod\bibinitdelim A\bibinitperiod}}}%
        {{hash=cb671e88fbe6c28dd80735f6227d7059}{%
           family={Behrens},
           familyi={B\bibinitperiod},
           given={Jess\bibnamedelima J},
           giveni={J\bibinitperiod\bibinitdelim J\bibinitperiod}}}%
        {{hash=b94ece5719ca6bb41b96b5b30667bcdc}{%
           family={Goel},
           familyi={G\bibinitperiod},
           given={Satyender},
           giveni={S\bibinitperiod}}}%
        {{hash=50ff34d43dcbb8730802cddfa30ee14e}{%
           family={Molitch},
           familyi={M\bibinitperiod},
           given={Mark\bibnamedelima E},
           giveni={M\bibinitperiod\bibinitdelim E\bibinitperiod}}}%
        {{hash=20a18291bfb11419b26ee7fa7e757f66}{%
           family={Kho},
           familyi={K\bibinitperiod},
           given={Abel\bibnamedelima N},
           giveni={A\bibinitperiod\bibinitdelim N\bibinitperiod}}}%
        {{hash=b0c9819ea01ef9c4e0b44094f76cc23a}{%
           family={Wallia},
           familyi={W\bibinitperiod},
           given={Amisha},
           giveni={A\bibinitperiod}}}%
      }
      \list{publisher}{1}{%
        {American Diabetes Association}%
      }
      \strng{namehash}{d2fb06a6de6e307b80795962545aa173}
      \strng{fullhash}{dd35435617843182daad4b964e995f13}
      \strng{bibnamehash}{d2fb06a6de6e307b80795962545aa173}
      \strng{authorbibnamehash}{d2fb06a6de6e307b80795962545aa173}
      \strng{authornamehash}{d2fb06a6de6e307b80795962545aa173}
      \strng{authorfullhash}{dd35435617843182daad4b964e995f13}
      \field{sortinit}{4}
      \field{sortinithash}{9381316451d1b9788675a07e972a12a7}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{journaltitle}{Diabetes Care}
      \field{number}{10}
      \field{title}{An evaluation of recurrent diabetic ketoacidosis, fragmentation of care, and mortality across Chicago, Illinois}
      \field{volume}{39}
      \field{year}{2016}
      \field{pages}{1671\bibrangedash 1676}
      \range{pages}{6}
    \endentry
    \entry{trick2021joining}{misc}{}
      \name{author}{6}{}{%
        {{hash=9533a43ff9aef61211dfcb9eae374860}{%
           family={Trick},
           familyi={T\bibinitperiod},
           given={William\bibnamedelima E},
           giveni={W\bibinitperiod\bibinitdelim E\bibinitperiod}}}%
        {{hash=febfb0a3417b6146fba6862c1d52e513}{%
           family={Hill},
           familyi={H\bibinitperiod},
           given={Jennifer\bibnamedelima C},
           giveni={J\bibinitperiod\bibinitdelim C\bibinitperiod}}}%
        {{hash=81da0956bc6ff0870defef3c8491c8cd}{%
           family={Toepfer},
           familyi={T\bibinitperiod},
           given={Peter},
           giveni={P\bibinitperiod}}}%
        {{hash=3884597145184959060c8ce2fb01bd67}{%
           family={Rachman},
           familyi={R\bibinitperiod},
           given={Fred},
           giveni={F\bibinitperiod}}}%
        {{hash=9c4372f2de5ed77e076236a2488cf068}{%
           family={Horwitz},
           familyi={H\bibinitperiod},
           given={Beth},
           giveni={B\bibinitperiod}}}%
        {{hash=0dbd1ac6692c980d1ce0e82c8ab5c475}{%
           family={Kho},
           familyi={K\bibinitperiod},
           given={Abel},
           giveni={A\bibinitperiod}}}%
      }
      \list{publisher}{1}{%
        {American Public Health Association}%
      }
      \strng{namehash}{644a5698987507e53571d61b1f72b7b2}
      \strng{fullhash}{4ceecd61d3ec7134a22a24476579f381}
      \strng{bibnamehash}{644a5698987507e53571d61b1f72b7b2}
      \strng{authorbibnamehash}{644a5698987507e53571d61b1f72b7b2}
      \strng{authornamehash}{644a5698987507e53571d61b1f72b7b2}
      \strng{authorfullhash}{4ceecd61d3ec7134a22a24476579f381}
      \field{sortinit}{4}
      \field{sortinithash}{9381316451d1b9788675a07e972a12a7}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{journaltitle}{American journal of public health}
      \field{number}{8}
      \field{title}{Joining Health Care and Homeless Data Systems Using Privacy-Preserving Record-Linkage Software}
      \field{volume}{111}
      \field{year}{2021}
      \field{pages}{1400\bibrangedash 1403}
      \range{pages}{4}
    \endentry
    \entry{walunas2017disease}{article}{}
      \name{author}{7}{}{%
        {{hash=9a1622e3e11f2d8588d8ae3ccff15c03}{%
           family={Walunas},
           familyi={W\bibinitperiod},
           given={Theresa\bibnamedelima L},
           giveni={T\bibinitperiod\bibinitdelim L\bibinitperiod}}}%
        {{hash=04040fd5e4bb8058acaeb3840a13db55}{%
           family={Jackson},
           familyi={J\bibinitperiod},
           given={Kathryn\bibnamedelima L},
           giveni={K\bibinitperiod\bibinitdelim L\bibinitperiod}}}%
        {{hash=ba1ee4e92e3f30ed789f135e35eefd5d}{%
           family={Chung},
           familyi={C\bibinitperiod},
           given={Anh\bibnamedelima H},
           giveni={A\bibinitperiod\bibinitdelim H\bibinitperiod}}}%
        {{hash=030a39b9230b9d0f29149d991c742da4}{%
           family={Mancera-Cuevas},
           familyi={M\bibinithyphendelim C\bibinitperiod},
           given={Karen\bibnamedelima A},
           giveni={K\bibinitperiod\bibinitdelim A\bibinitperiod}}}%
        {{hash=44a4661749dee19983c31cdf40d87128}{%
           family={Erickson},
           familyi={E\bibinitperiod},
           given={Daniel\bibnamedelima L},
           giveni={D\bibinitperiod\bibinitdelim L\bibinitperiod}}}%
        {{hash=2ece4101c34c6411097deb3c87229fae}{%
           family={Ramsey-Goldman},
           familyi={R\bibinithyphendelim G\bibinitperiod},
           given={Rosalind},
           giveni={R\bibinitperiod}}}%
        {{hash=0dbd1ac6692c980d1ce0e82c8ab5c475}{%
           family={Kho},
           familyi={K\bibinitperiod},
           given={Abel},
           giveni={A\bibinitperiod}}}%
      }
      \list{publisher}{1}{%
        {Wiley Online Library}%
      }
      \strng{namehash}{8ac72442d48b4d6e33021afc592ec4c0}
      \strng{fullhash}{cbcdf5967018e02b121faf83f337ba1a}
      \strng{bibnamehash}{8ac72442d48b4d6e33021afc592ec4c0}
      \strng{authorbibnamehash}{8ac72442d48b4d6e33021afc592ec4c0}
      \strng{authornamehash}{8ac72442d48b4d6e33021afc592ec4c0}
      \strng{authorfullhash}{cbcdf5967018e02b121faf83f337ba1a}
      \field{sortinit}{4}
      \field{sortinithash}{9381316451d1b9788675a07e972a12a7}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{journaltitle}{Arthritis care \& research}
      \field{number}{9}
      \field{title}{Disease outcomes and care fragmentation among patients with systemic lupus erythematosus}
      \field{volume}{69}
      \field{year}{2017}
      \field{pages}{1369\bibrangedash 1376}
      \range{pages}{8}
    \endentry
    \entry{mraia}{misc}{}
      \name{author}{1}{}{%
        {{hash=e0bb64de5329ff83f03383222a481f51}{%
           family={{Medical Research Analytics and Informatics Alliance}},
           familyi={M\bibinitperiod}}}%
      }
      \strng{namehash}{e0bb64de5329ff83f03383222a481f51}
      \strng{fullhash}{e0bb64de5329ff83f03383222a481f51}
      \strng{bibnamehash}{e0bb64de5329ff83f03383222a481f51}
      \strng{authorbibnamehash}{e0bb64de5329ff83f03383222a481f51}
      \strng{authornamehash}{e0bb64de5329ff83f03383222a481f51}
      \strng{authorfullhash}{e0bb64de5329ff83f03383222a481f51}
      \field{sortinit}{5}
      \field{sortinithash}{20e9b4b0b173788c5dace24730f47d8c}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{howpublished}{\url{https://www.mraia.org}}
      \field{note}{Accessed: 2022-02-25}
      \field{title}{Public health and research informatics}
    \endentry
    \entry{Bater2017}{article}{}
      \name{author}{6}{}{%
        {{hash=01dac0b9558906afccda30a5a76caee6}{%
           family={Bater},
           familyi={B\bibinitperiod},
           given={Johes},
           giveni={J\bibinitperiod}}}%
        {{hash=cf3ac60ba706bfbd56bfa7c6e0dbcf14}{%
           family={Elliott},
           familyi={E\bibinitperiod},
           given={Gregory},
           giveni={G\bibinitperiod}}}%
        {{hash=ee1579761934ae726e60f8e2a92a72e7}{%
           family={Eggen},
           familyi={E\bibinitperiod},
           given={Craig},
           giveni={C\bibinitperiod}}}%
        {{hash=b94ece5719ca6bb41b96b5b30667bcdc}{%
           family={Goel},
           familyi={G\bibinitperiod},
           given={Satyender},
           giveni={S\bibinitperiod}}}%
        {{hash=0dbd1ac6692c980d1ce0e82c8ab5c475}{%
           family={Kho},
           familyi={K\bibinitperiod},
           given={Abel},
           giveni={A\bibinitperiod}}}%
        {{hash=6ad6d6c3824f59ddd5677a25fac9f9a7}{%
           family={Rogers},
           familyi={R\bibinitperiod},
           given={Jennie},
           giveni={J\bibinitperiod}}}%
      }
      \strng{namehash}{9d687e2ddc778c8c1471b23e770376ef}
      \strng{fullhash}{d29c4d6b906d4136268cfd10fed68ac2}
      \strng{bibnamehash}{9d687e2ddc778c8c1471b23e770376ef}
      \strng{authorbibnamehash}{9d687e2ddc778c8c1471b23e770376ef}
      \strng{authornamehash}{9d687e2ddc778c8c1471b23e770376ef}
      \strng{authorfullhash}{d29c4d6b906d4136268cfd10fed68ac2}
      \field{extraname}{1}
      \field{sortinit}{6}
      \field{sortinithash}{b33bc299efb3c36abec520a4c896a66d}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{issn}{21508097}
      \field{journaltitle}{PVLDB}
      \field{number}{6}
      \field{title}{{SMCQL: secure querying for federated databases}}
      \field{volume}{10}
      \field{year}{2017}
      \field{pages}{673\bibrangedash 684}
      \range{pages}{12}
      \verb{doi}
      \verb 10.14778/3055330.3055334
      \endverb
    \endentry
    \entry{galanter2013migration}{article}{}
      \name{author}{10}{}{%
        {{hash=0381083961cc77da1013ca2a3970ace3}{%
           family={Galanter},
           familyi={G\bibinitperiod},
           given={William\bibnamedelima L},
           giveni={W\bibinitperiod\bibinitdelim L\bibinitperiod}}}%
        {{hash=c3c47ce77237cea8fe59960c9bc786dc}{%
           family={Applebaum},
           familyi={A\bibinitperiod},
           given={Andrew},
           giveni={A\bibinitperiod}}}%
        {{hash=12a06b05d45390e963aaa1af22168c33}{%
           family={Boddipalli},
           familyi={B\bibinitperiod},
           given={Viveka},
           giveni={V\bibinitperiod}}}%
        {{hash=0dbd1ac6692c980d1ce0e82c8ab5c475}{%
           family={Kho},
           familyi={K\bibinitperiod},
           given={Abel},
           giveni={A\bibinitperiod}}}%
        {{hash=db7be6d0564aa601a63307dc5039fe35}{%
           family={Lin},
           familyi={L\bibinitperiod},
           given={Michael},
           giveni={M\bibinitperiod}}}%
        {{hash=14629b0cfc0ba33d41f7a8dd053c0632}{%
           family={Meltzer},
           familyi={M\bibinitperiod},
           given={David},
           giveni={D\bibinitperiod}}}%
        {{hash=97e50bfef3489022a123b161168c840d}{%
           family={Roberts},
           familyi={R\bibinitperiod},
           given={Anna},
           giveni={A\bibinitperiod}}}%
        {{hash=ed20fe7c3b5d9be544e12787f78f769f}{%
           family={Trick},
           familyi={T\bibinitperiod},
           given={Bill},
           giveni={B\bibinitperiod}}}%
        {{hash=261af5b444d46ff3869c0e9ac305bdb1}{%
           family={Walton},
           familyi={W\bibinitperiod},
           given={Surrey\bibnamedelima M},
           giveni={S\bibinitperiod\bibinitdelim M\bibinitperiod}}}%
        {{hash=57eb15805587927f638828d905b8b2c4}{%
           family={Lambert},
           familyi={L\bibinitperiod},
           given={Bruce\bibnamedelima L},
           giveni={B\bibinitperiod\bibinitdelim L\bibinitperiod}}}%
      }
      \list{publisher}{1}{%
        {Springer}%
      }
      \strng{namehash}{05e9050efa798f334db8a953d85c6f31}
      \strng{fullhash}{3054b6838f0c3165bb07a9a3d43fc531}
      \strng{bibnamehash}{05e9050efa798f334db8a953d85c6f31}
      \strng{authorbibnamehash}{05e9050efa798f334db8a953d85c6f31}
      \strng{authornamehash}{05e9050efa798f334db8a953d85c6f31}
      \strng{authorfullhash}{3054b6838f0c3165bb07a9a3d43fc531}
      \field{sortinit}{6}
      \field{sortinithash}{b33bc299efb3c36abec520a4c896a66d}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{journaltitle}{Journal of medical systems}
      \field{number}{2}
      \field{title}{Migration of patients between five urban teaching hospitals in Chicago}
      \field{volume}{37}
      \field{year}{2013}
      \field{pages}{1\bibrangedash 8}
      \range{pages}{8}
    \endentry
    \entry{Bater2018}{article}{}
      \name{author}{5}{}{%
        {{hash=01dac0b9558906afccda30a5a76caee6}{%
           family={Bater},
           familyi={B\bibinitperiod},
           given={Johes},
           giveni={J\bibinitperiod}}}%
        {{hash=5ca5eefe97141a92dff9eb1a1b3e0d49}{%
           family={He},
           familyi={H\bibinitperiod},
           given={Xi},
           giveni={X\bibinitperiod}}}%
        {{hash=9fc15e0207741a7b705b6cb83557120b}{%
           family={Ehrich},
           familyi={E\bibinitperiod},
           given={William},
           giveni={W\bibinitperiod}}}%
        {{hash=3fb56c38e8253a373656e279a5cd89da}{%
           family={Machanavajjhala},
           familyi={M\bibinitperiod},
           given={Ashwin},
           giveni={A\bibinitperiod}}}%
        {{hash=6ad6d6c3824f59ddd5677a25fac9f9a7}{%
           family={Rogers},
           familyi={R\bibinitperiod},
           given={Jennie},
           giveni={J\bibinitperiod}}}%
      }
      \list{publisher}{1}{%
        {VLDB Endowment}%
      }
      \strng{namehash}{9d687e2ddc778c8c1471b23e770376ef}
      \strng{fullhash}{d32d960ae3258608fe72a6a514802f13}
      \strng{bibnamehash}{d32d960ae3258608fe72a6a514802f13}
      \strng{authorbibnamehash}{d32d960ae3258608fe72a6a514802f13}
      \strng{authornamehash}{9d687e2ddc778c8c1471b23e770376ef}
      \strng{authorfullhash}{d32d960ae3258608fe72a6a514802f13}
      \field{extraname}{2}
      \field{sortinit}{7}
      \field{sortinithash}{108d0be1b1bee9773a1173443802c0a3}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{journaltitle}{PVLDB}
      \field{number}{3}
      \field{title}{Shrinkwrap: efficient SQL Query Processing in Differentially Private Data Federations}
      \field{volume}{12}
      \field{year}{2018}
      \field{pages}{307\bibrangedash 320}
      \range{pages}{14}
    \endentry
    \entry{bater2020saqe}{article}{}
      \name{author}{5}{}{%
        {{hash=01dac0b9558906afccda30a5a76caee6}{%
           family={Bater},
           familyi={B\bibinitperiod},
           given={Johes},
           giveni={J\bibinitperiod}}}%
        {{hash=fce20b8d3e68b8874ed9f95a28fd9d05}{%
           family={Park},
           familyi={P\bibinitperiod},
           given={Yongjoo},
           giveni={Y\bibinitperiod}}}%
        {{hash=5ca5eefe97141a92dff9eb1a1b3e0d49}{%
           family={He},
           familyi={H\bibinitperiod},
           given={Xi},
           giveni={X\bibinitperiod}}}%
        {{hash=bd7d15d79ca36b953d99a1a0aaccb94a}{%
           family={Wang},
           familyi={W\bibinitperiod},
           given={Xiao},
           giveni={X\bibinitperiod}}}%
        {{hash=6ad6d6c3824f59ddd5677a25fac9f9a7}{%
           family={Rogers},
           familyi={R\bibinitperiod},
           given={Jennie},
           giveni={J\bibinitperiod}}}%
      }
      \list{publisher}{1}{%
        {VLDB Endowment}%
      }
      \strng{namehash}{9d687e2ddc778c8c1471b23e770376ef}
      \strng{fullhash}{73a78e2eb04f49a1fac6fe81518fa8be}
      \strng{bibnamehash}{73a78e2eb04f49a1fac6fe81518fa8be}
      \strng{authorbibnamehash}{73a78e2eb04f49a1fac6fe81518fa8be}
      \strng{authornamehash}{9d687e2ddc778c8c1471b23e770376ef}
      \strng{authorfullhash}{73a78e2eb04f49a1fac6fe81518fa8be}
      \field{extraname}{3}
      \field{sortinit}{8}
      \field{sortinithash}{a231b008ebf0ecbe0b4d96dcc159445f}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{journaltitle}{Proceedings of the VLDB Endowment}
      \field{number}{12}
      \field{title}{{SAQE}: practical privacy-preserving approximate query processing for data federations}
      \field{volume}{13}
      \field{year}{2020}
      \field{pages}{2691\bibrangedash 2705}
      \range{pages}{15}
    \endentry
    \entry{4568207}{inproceedings}{}
      \name{author}{1}{}{%
        {{hash=bdf7dbd523c5db366c4ffbc0ea3dc192}{%
           family={Yao},
           familyi={Y\bibinitperiod},
           given={Andrew\bibnamedelima Chi-Chih},
           giveni={A\bibinitperiod\bibinitdelim C\bibinithyphendelim C\bibinitperiod}}}%
      }
      \strng{namehash}{bdf7dbd523c5db366c4ffbc0ea3dc192}
      \strng{fullhash}{bdf7dbd523c5db366c4ffbc0ea3dc192}
      \strng{bibnamehash}{bdf7dbd523c5db366c4ffbc0ea3dc192}
      \strng{authorbibnamehash}{bdf7dbd523c5db366c4ffbc0ea3dc192}
      \strng{authornamehash}{bdf7dbd523c5db366c4ffbc0ea3dc192}
      \strng{authorfullhash}{bdf7dbd523c5db366c4ffbc0ea3dc192}
      \field{sortinit}{9}
      \field{sortinithash}{0a5ebc79d83c96b6579069544c73c7d4}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{booktitle}{27th Annual Symposium on Foundations of Computer Science (FOCS 1986)}
      \field{title}{How to generate and exchange secrets}
      \field{year}{1986}
      \field{pages}{162\bibrangedash 167}
      \range{pages}{6}
      \verb{doi}
      \verb 10.1109/SFCS.1986.25
      \endverb
    \endentry
    \entry{emp-toolkit}{misc}{}
      \name{author}{3}{}{%
        {{hash=bd7d15d79ca36b953d99a1a0aaccb94a}{%
           family={Wang},
           familyi={W\bibinitperiod},
           given={Xiao},
           giveni={X\bibinitperiod}}}%
        {{hash=74c98a0cc6e77d8e1633c4ddc677de39}{%
           family={Malozemoff},
           familyi={M\bibinitperiod},
           given={Alex\bibnamedelima J.},
           giveni={A\bibinitperiod\bibinitdelim J\bibinitperiod}}}%
        {{hash=85053e14c4a72772970b91a572b9b9c1}{%
           family={Katz},
           familyi={K\bibinitperiod},
           given={Jonathan},
           giveni={J\bibinitperiod}}}%
      }
      \strng{namehash}{0d4d723537ce643363f661a0a7e6cce0}
      \strng{fullhash}{41b033a1fa7d2f14c850c6ca64c87245}
      \strng{bibnamehash}{41b033a1fa7d2f14c850c6ca64c87245}
      \strng{authorbibnamehash}{41b033a1fa7d2f14c850c6ca64c87245}
      \strng{authornamehash}{0d4d723537ce643363f661a0a7e6cce0}
      \strng{authorfullhash}{41b033a1fa7d2f14c850c6ca64c87245}
      \field{sortinit}{1}
      \field{sortinithash}{4f6aaa89bab872aa0999fec09ff8e98a}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{howpublished}{\url{https://github.com/emp-toolkit}}
      \field{title}{{EMP-toolkit: Efficient Multiparty computation toolkit}}
      \field{year}{2016}
    \endentry
    \entry{preventionDP1815}{misc}{}
      \name{author}{1}{}{%
        {{hash=3b242b66dfe956017e7e4b5d73d0c164}{%
           family={{Centers for Disease Control and Prevention}},
           familyi={C\bibinitperiod}}}%
      }
      \strng{namehash}{3b242b66dfe956017e7e4b5d73d0c164}
      \strng{fullhash}{3b242b66dfe956017e7e4b5d73d0c164}
      \strng{bibnamehash}{3b242b66dfe956017e7e4b5d73d0c164}
      \strng{authorbibnamehash}{3b242b66dfe956017e7e4b5d73d0c164}
      \strng{authornamehash}{3b242b66dfe956017e7e4b5d73d0c164}
      \strng{authorfullhash}{3b242b66dfe956017e7e4b5d73d0c164}
      \field{sortinit}{1}
      \field{sortinithash}{4f6aaa89bab872aa0999fec09ff8e98a}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{howpublished}{\url{https://www.cdc.gov/diabetes/programs/stateandlocal/funded-programs/dp18-1815.html}}
      \field{title}{{DP18-1815}: Improving the Health of Americans Through Prevention and Management of Diabetes, Heart Disease, and Stroke}
    \endentry
    \entry{ahmad2019challenges}{article}{}
      \true{moreauthor}
      \true{morelabelname}
      \name{author}{10}{}{%
        {{hash=fee40ce69a9b772ddcee95a8553ad2e4}{%
           family={Ahmad},
           familyi={A\bibinitperiod},
           given={Faraz\bibnamedelima S},
           giveni={F\bibinitperiod\bibinitdelim S\bibinitperiod}}}%
        {{hash=c5ddf8425f10666f00d2b8dc9ee9cb59}{%
           family={Rasmussen},
           familyi={R\bibinitperiod},
           given={Luke\bibnamedelima V},
           giveni={L\bibinitperiod\bibinitdelim V\bibinitperiod}}}%
        {{hash=5b49613275c32f237e67ed10f88e5b57}{%
           family={Persell},
           familyi={P\bibinitperiod},
           given={Stephen\bibnamedelima D},
           giveni={S\bibinitperiod\bibinitdelim D\bibinitperiod}}}%
        {{hash=f38e79494519c59c4f965c775837782e}{%
           family={Richardson},
           familyi={R\bibinitperiod},
           given={Joshua\bibnamedelima E},
           giveni={J\bibinitperiod\bibinitdelim E\bibinitperiod}}}%
        {{hash=39101af4fd00a4c527216f606a45c506}{%
           family={Liss},
           familyi={L\bibinitperiod},
           given={David\bibnamedelima T},
           giveni={D\bibinitperiod\bibinitdelim T\bibinitperiod}}}%
        {{hash=c75d5bd40ae9f2884b61178df50a2657}{%
           family={Kenly},
           familyi={K\bibinitperiod},
           given={Pauline},
           giveni={P\bibinitperiod}}}%
        {{hash=6e1464bdcfb6583518e1187b65961521}{%
           family={Chung},
           familyi={C\bibinitperiod},
           given={Isabel},
           giveni={I\bibinitperiod}}}%
        {{hash=948e85acaea8ecde8f0a5cd66d8472a9}{%
           family={French},
           familyi={F\bibinitperiod},
           given={Dustin\bibnamedelima D},
           giveni={D\bibinitperiod\bibinitdelim D\bibinitperiod}}}%
        {{hash=9a1622e3e11f2d8588d8ae3ccff15c03}{%
           family={Walunas},
           familyi={W\bibinitperiod},
           given={Theresa\bibnamedelima L},
           giveni={T\bibinitperiod\bibinitdelim L\bibinitperiod}}}%
        {{hash=1ab7ebe682d8f3669f73652e240a700e}{%
           family={Schriever},
           familyi={S\bibinitperiod},
           given={Andy},
           giveni={A\bibinitperiod}}}%
      }
      \list{publisher}{1}{%
        {Oxford University Press}%
      }
      \strng{namehash}{f8f75af7b04481f2d7ef83fccfb2c765}
      \strng{fullhash}{f4962522ef7930b4d3819738599e6449}
      \strng{bibnamehash}{f8f75af7b04481f2d7ef83fccfb2c765}
      \strng{authorbibnamehash}{f8f75af7b04481f2d7ef83fccfb2c765}
      \strng{authornamehash}{f8f75af7b04481f2d7ef83fccfb2c765}
      \strng{authorfullhash}{f4962522ef7930b4d3819738599e6449}
      \field{sortinit}{1}
      \field{sortinithash}{4f6aaa89bab872aa0999fec09ff8e98a}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{journaltitle}{JAMIA open}
      \field{number}{4}
      \field{title}{Challenges to electronic clinical quality measurement using third-party platforms in primary care practices: the healthy hearts in the heartland experience}
      \field{volume}{2}
      \field{year}{2019}
      \field{pages}{423\bibrangedash 428}
      \range{pages}{6}
    \endentry
    \entry{datavant}{misc}{}
      \field{sortinit}{1}
      \field{sortinithash}{4f6aaa89bab872aa0999fec09ff8e98a}
      \field{labeltitlesource}{title}
      \field{howpublished}{\url{https://datavant.com}}
      \field{note}{Accessed: 2022-02-25}
      \field{title}{{Datavant: Connecting Health Data to Improve Patient Outcomes}}
    \endentry
    \entry{harinarayan1996implementing}{article}{}
      \name{author}{3}{}{%
        {{hash=a18962cfee6eb4e3108254f802ee658a}{%
           family={Harinarayan},
           familyi={H\bibinitperiod},
           given={Venky},
           giveni={V\bibinitperiod}}}%
        {{hash=45500b3dfad3d2cf0ce07cd00149af68}{%
           family={Rajaraman},
           familyi={R\bibinitperiod},
           given={Anand},
           giveni={A\bibinitperiod}}}%
        {{hash=cafe1d770c56825ebccdb81e9f7c9b3b}{%
           family={Ullman},
           familyi={U\bibinitperiod},
           given={Jeffrey\bibnamedelima D},
           giveni={J\bibinitperiod\bibinitdelim D\bibinitperiod}}}%
      }
      \list{publisher}{1}{%
        {ACM New York, NY, USA}%
      }
      \strng{namehash}{0f7a4479e600f84f5c1e407949ad8d01}
      \strng{fullhash}{a147b4cbbf47d18def999434b7701122}
      \strng{bibnamehash}{a147b4cbbf47d18def999434b7701122}
      \strng{authorbibnamehash}{a147b4cbbf47d18def999434b7701122}
      \strng{authornamehash}{0f7a4479e600f84f5c1e407949ad8d01}
      \strng{authorfullhash}{a147b4cbbf47d18def999434b7701122}
      \field{sortinit}{1}
      \field{sortinithash}{4f6aaa89bab872aa0999fec09ff8e98a}
      \field{labelnamesource}{author}
      \field{labeltitlesource}{title}
      \field{journaltitle}{Acm Sigmod Record}
      \field{number}{2}
      \field{title}{Implementing data cubes efficiently}
      \field{volume}{25}
      \field{year}{1996}
      \field{pages}{205\bibrangedash 216}
      \range{pages}{12}
    \endentry
  \enddatalist
\endrefsection
\endinput


